Automatically Recommend Code Updates: Are We There Yet?

In recent years, large pre-trained Language Models of Code (CodeLMs) have shown promising results on various software engineering tasks. One such task is automatic code update recommendation, which transforms outdated code snippets into their approved and revised counterparts. Although many CodeLM-based approaches have been proposed, claiming high accuracy, their effectiveness and reliability on real-world code update tasks remain questionable. In this paper, we present the first extensive evaluation of state-of-the-art CodeLMs for automatically recommending code updates. We assess their performance on two diverse datasets of paired updated methods, considering factors such as temporal evolution, project specificity, method size, and update complexity. Our results reveal that while CodeLMs perform well in settings that ignore temporal information, they struggle in more realistic time-wise scenarios and generalize poorly to new projects. Furthermore, CodeLM performance decreases significantly for larger methods and more complex updates. Furthermore, we observe that many CodeLM-generated "updates" are actually null, especially in time-wise settings, and meaningful edits remain challenging. Our findings highlight the significant gap between the perceived and actual effectiveness of CodeLMs for real-world code update recommendation and emphasize the need for more research on improving their practicality, robustness, and generalizability.

==> history/result.tex <==
\section{Experimental Results}
\label{sec:results} 

In this section, we present approaches and results with respect to our five research questions.



\subsection*{\textbf{(RQ1) \rqone}}
% \pick{We also have a result for efficiency. Should RQ be adjusted to include efficiency?}
\paragraph{\textbf{\underline{Motivation}}}
This research question aims to investigate the accuracy of our proposed approach, \ourapp~(CodeT5), in the context of code recommendation in Android apps, compared to two baseline code transformation approaches and other four pre-trained NLMs approaches.
By evaluating the accuracy, we aim to demonstrate the effectiveness of \ourapp~in generating suitable code recommendations.

\paragraph{\textbf{\underline{Approach}}}
To answer this RQ, we evaluate the accuracy of \ourapp~ and the baseline approaches by calculating the percentage of Perfect Predictions (\%PP). %, BLEU, and CodeBLEU.
Following the methodology of previous studies~\cite{tufano2019learning,thongtanunam2022autotransform}, we employ a beam search with beam widths ($k$) of 1, 5, 10, and 15 to generate $k$ candidate code updates.
To determine the extent of the improvement achieved by \ourapp, we compute the percentage improvement in the perfect predictions rate using the formula: $\frac{(\#PP\%_\mathrm{our} - \#PP\%_\mathrm{baseline})\times 100\%}{\#PP\%_\mathrm{baseline}}$. Furthermore, we also compare \ourapp~ with the baseline approaches based on the BLEU and CodeBLEU metrics, which offer additional insights into the quality and similarity of the generated code updates compared to the ground truth.

 
It is important to note that the RNN architecture employed by the baseline approaches~\cite{tufano2019learning} is computationally expensive, leading to the evaluation of these approaches using small methods only (i.e., those with fewer than 50 tokens in a method and fewer than 5 changed tokens between versions).
Consequently, in line with prior studies~\cite{tufano2019learning, thongtanunam2022autotransform}, our analysis in this research question will be focused on the context of small methods.
For each approach, the model is trained on the training dataset consisting of small methods and tested on the corresponding testing dataset of small methods. 
This approach enables us to maintain consistency with previous studies, allowing for a fair comparison of \ourapp~ with the baseline methods. 
In a subsequent research question (RQ4), we will extend our evaluation to encompass the entire dataset, providing a more comprehensive assessment of \ourapp~ in various contexts and code update scenarios.

\input{tables/RQ1_compare_with_baseline}

\paragraph{\textbf{\underline{Results}}}
\textbf{\ourapp~ achieves a perfect prediction of 31\%, which is 190\%\textasciitilde385\% higher than the baseline approaches.}
Table~\ref{tab:RQ1compare} compares the accuracy of \ourapp~ to two baseline approaches, Tufano \ea~ and AutoTransform.
We observe that \ourapp~ significantly outperforms these methods in terms of perfect prediction percentages. 
When the beam size is set to 15, \ourapp~ achieves perfect predictions for 31\% of the changed methods (1916 out of the total).
In contrast, Tufano \ea~ achieves a perfect prediction rate of 6\% (277 changed methods), while AutoTransform has a rate of 11\% (661 changed methods). 
This corresponds to a 385\% performance improvement over Tufano \ea~ and a 190\% improvement over AutoTransform.
For beam sizes of 1, 5, or 10, \ourapp~ also demonstrates substantial improvements in perfect prediction rates, ranging from 343\% to 432\% when compared to Tufano \ea~ and 110\% to 179\% when compared to AutoTransform. 
These observations demonstrate that \ourapp~ outperforms Tufano \ea~ and AutoTransform to generate a perfect prediction by a large margin. 

In addition to perfect predictions, \ourapp~ consistently achieves higher BLEU and CodeBLEU scores than the baseline approaches across all beam sizes. 
For example, when the beam size is set to 15, \ourapp~ attains a CodeBLEU score of 0.88, whereas Tufano \ea~ and AutoTransform achieve scores of 0.75 and 0.87, espectively. 
This pattern is maintained for beam sizes of 1, 5, and 10, indicating that \ourapp~ can generate code updates more similar to the actual updates on average across all tested methods.
Overall, these results demonstrate the considerable benefits of employing pre-trained NLMs in \ourapp~ for achieving superior performance compared to traditional baseline approaches.


\textbf{\ourapp~ demonstrates competitive performance in comparison to other pre-trained models.}
When examining the performance of \ourapp~ against other pre-trained models such as CodeBERT, CodeGPT, UniXcoder and T5, we observe that \ourapp~ consistently achieves a higher perfect prediction percentage across all beam sizes. 
Specifically, when the beam size is set to 15, \ourapp~ achieves a 31\% perfect prediction rate, while CodeBERT reaches only 12\%, CodeGPT only 18\%, and UniXcoder only 17\%.
Similar trends are observed for beam sizes of 1, 5, and 10, where \ourapp~ persistently outperforms the other pre-trained models in terms of perfect prediction rate, BLEU and CodeBLEU scores.
These results suggest that compared with other NLMs, CodeT5 can be more effective for automated code recommendations.
Additionally, we discovered that CodeT5 can improve the performance of T5 from 25\% to 31\%. 
Although CodeT5 is based on the T5 architecture, the results indicate that domain-specific pre-training have significantly contributed to its enhanced performance in code recommendation tasks.



% \textbf{Our \ourapp~ achieves a higher efficiency for recommending code updates compared with the Tufano~\ea~approach and AutoTransform.}
% Table~\ref{tab:RQ1timecompare} shows the computational time of our \ourapp{} and the baseline approaches.
% As shown in Table~\ref{tab:RQ1timecompare}, \ourapp~ takes about 117 minutes to train a model, while the approach of Tufano \ea~ takes 223 minutes and AutoTransform takes 140 minutes.
% The result shows that our \ourapp~ can save 16\% - 50\% computational time when training a model on the small dataset. 
% The higher efficiency of our \ourapp~has to do with our Transformer-based architecture, which processes the entire input sequences at once in a highly parallel fashion. 
% In contrast, the RNNs-based models used by Tufano~\ea~\cite{tufano2019learning} needs to process the input sequence in order, which is less efficient as showed in Table~\ref{tab:RQ1timecompare}.

% \yonghui{Do we need to mention why higher efficiency than AutoTransform?}
% \kla{may be no because both autoupdate and autotransform use the same architecture, but we do not have reason to support why autoupdate is faster than autotransform}
% \pick{Please a short discussion why it takes less time to compute? The vocab size is smaller?}


\begin{table}[htbp]
  \centering
  \small
  \caption{Computational time of \ourapp~ and the baseline approaches.}
    \begin{tabular}{lrrr}
    \toprule
    \textbf{ Model } & \multicolumn{1}{c}{\textbf{ \ourapp }} & \multicolumn{1}{c}{\textbf{ Tufano \ea }} & \multicolumn{1}{c}{\textbf{ AutoTransform }} \\
    \midrule
    \textbf{Time cost} & 117 min & 233 min & 140 min \\
    \textbf{Improvement} &       & -50\% & -16\% \\
    \bottomrule
    \end{tabular}%
  \label{tab:RQ1timecompare}%
\end{table}%





\subsection*{\textbf{(RQ2) \rqtwo}}

\paragraph{\textbf{\underline{Motivation}}} 
Tufano~\ea~\cite{tufano2019learning} suggested that code abstraction could substantially reduce the size of vocabularies. 
However, Thongtanunam~\ea~\cite{thongtanunam2022autotransform} argue that, when code abstraction is used together with word-level tokenization, the approach may generate an excessively large number of vocabularies.
Different from prior work, our \ourapp~leverages both code abstraction and BPE in order to preserve existing tokens that will be appeared in the updated version and generate new tokens that do not exist in the prior version.
Thus, we formulate this RQ to investigate the benefits of our tokenization approaches for our \ourapp.

\paragraph{\textbf{\underline{Approach}}}
To answer this RQ, we conduct an ablation study to evaluate the following four variants of our \ourapp~ using different tokenization approaches:

\begin{itemize}
    \item Abs+BPE+Transformer (our \ourapp).
    \item BPE+Transformer (AutoTransform~\cite{thongtanunam2022autotransform}).
    \item Abs+Transformer (Abs is used in Tufano~\ea~\cite{tufano2019learning}).
    \item Word-level+Transformer.
\end{itemize}
Similar to RQ1, for each approach, the model is trained on the training dataset of small methods and tested on the testing dataset of small methods.
Finally, we evaluate the accuracy of these variants using the same evaluation measure (i.e., \% Perfect Predictions).


% To answer this RQ, we conduct an experiment of different code tokenization approach with the same Transformer architecture. 
% Specifically, we extend our approaches to evaluate the following four variants: word-based tokenization (i.e., 1-gram word level tokenization which splits raw code by white space), only code abstraction, only BPE subword toknization, and code abstraction + BPE. 
% After that, we build the Transformer to test the prediction performance. 
% We evaluate the accuracy (i.e., perfect prediction rate) under different beam sizes.

\begin{figure}[t]
  \centering
  \includegraphics[width=0.8\columnwidth]{results/RQ2.pdf}
  \caption{(RQ2) The perfect prediction of the different tokenization approaches.}
  \label{fig:RQ2Evaluation_tokenization}
\end{figure}


\paragraph{\textbf{\underline{Results}}}
Figure~\ref{fig:RQ2Evaluation_tokenization} presents the accuracy of different code tokenization approaches of our \ourapp.

\textbf{Our tokenization approach (Abs + BPE) gains benefits at least 17\% by using both code abstraction and BPE for recommending code updates.}
Figure~\ref{fig:RQ2Evaluation_tokenization} shows that our approach (Abs + BPE) achieves the highest accuracy regardless of the size of beam search.
Specifically, at the beam size of 15, our approach achieves the perfect prediction of 25\%.
On the other hand, code abstraction alone achieves the perfect prediction of 23\%, while BPE alone achieves the perfect prediction of 11\%.
The higher accuracy of using code abstraction only than using BPE only is different from Thongtanunam~\ea~\cite{thongtanunam2022autotransform} who found that BPE is better than code abstraction, highlighting the importance of this work that findings from existing NMT-based code transformation studies are not generalized to NMT-based code update recommendations.
We suspect that BPE works well for the context of code review, since there are a large number of newly-introduced code tokens.
In contrast, for Android apps, the proportion of newly-introduced code tokens is smaller, demonstrating that code abstraction only performs better than BPE only.
Nevertheless, our finding confirms that the combination of using both Abs and BPE used by our \ourapp~outperforms both Abs alone and BPE alone.


\subsection*{\textbf{(RQ3) \rqthree}}

\paragraph{\textbf{\underline{Motivation}}}
Prior studies proposed various approaches to automatically update Android apps, yet for specific types of code updates.
For example, 
Lamothe et al.~\cite{lamothe2020a3} focus on updating Android API migrations.
Zhao et al.~\cite{zhao2022towards} focus on updating compatibility issues.
% However, existing approaches are .
Indeed, there exist multiple types of code updates~\cite{Conventional-commit-types} associated with Android apps (e.g., \textit{Fixing Bug} or \textit{Refactoring Method}).
Thus, we set out this RQ to qualitatively evaluate \ourapp{} in terms of the types of code updates that can be recommended by our \ourapp. 


\paragraph{\textbf{\underline{Approach}}}
To answer this RQ, we analyze the 277 updated methods that are correctly recommended by our \ourapp{} when using the beam size of 1 from RQ1.
% ~(i.e., the group of 7\% perfect predictions at the beam size of 1).
To do so, we manually classify updated methods into various types of code updates. 
% \lili{The next sentence is not correct.}
We use the high-level taxonomy of the conventional commit types~\cite{Conventional-commit-types} and Tufano~\ea's approach~\cite{tufano2019learning} for the types of code updates. 
To fully understand the purpose of code updates, we also use the commit messages associated with the studied updated methods. 
% For each of the method pairs, we collect the human-written commit log messages that are associated with that method pair.
% Commit messages are natural language descriptions of changes in source code written by software developers, which is often used to describe the intent of the code changes, e.g., "\emph{Fix integer division in floating-point contexts}".
The categorization process was performed by the first author and the results of coding were cross-checked by the third author to mitigate any potential bias in the categorization process.
Then, we calculate the inter-rater agreement between the categorization results from the two coders using a Cohen's kappa. 
The kappa agreement is 0.91 for the categorization process of the 277 perfect predictions, demonstrating the high agreement (i.e., almost perfect) between two raters~\cite{cohen1968weighted}.



\paragraph{\textbf{\underline{Results}}} 
% \kla{@Li, can check below?}
Table~\ref{tab:rq5} sumarizes the types of code updates that  our \ourapp{} can achieve concerning a perfect prediction with a beam size of 1.\footnote{Due to the page limit, the complete classification results are available in the GitHub repository.}

\textbf{Our \ourapp~ can recommend nine types of code updates for Android apps, e.g., 26\% perfect predictions for fixing bug and 22\% perfect predictions for adding new features.}
As Table~\ref{tab:rq5} shows, we summarize nine types of code updates.
\textit{Fixing bug} and \textit{Adding New Feature} are the most common types of code updates that \ourapp{} can recommend (i.e., 26\% for \textit{Fixing Bug} and 22\% for \textit{Adding New Feature}).
Also, our \ourapp{} can recommend maintainability-related code updates for Android applications (e.g., \textit{Refactoring Method} and \textit{Adjusting Build} for Android applications).
Additionally, some of the code updates are related to external code updates (e.g., third-party libraries and Android OS).
For example, Android developers update the source code to adapt to the release of new version of Android OS (i.e., Maintaining Android OS Compatibility).
% Another example is that Android developers need to update the source code to accommodate the new third-party libraries (i.e., \pick{what type?}). 
These results suggest that our \ourapp{} can recommend various types of code updates, demonstrating the potential impact of our \ourapp{} in real-world usage scenarios.



\input{tables/RQ5}

\subsection*{\textbf{(RQ4) \rqfour}}

\paragraph{\textbf{\underline{Motivation}}}
Source codes gradually evolves over time.
Thus, evaluation scenarios for NMT-based code transformation should take into consideration temporal information. 
Prior studies~\cite{pornprasit2021jitline,cabral2019class, pendlebury2019tesseract, de2021compromised} raised concerns that random data splitting (which has been widely-used in previous NMT-based code transformation approaches~\cite{tufano2018empirical,thongtanunam2022autotransform}) may not be realistic (i.e., time-ignore), ignoring the temporal information that must be considered.
Yet, little is known about the impact of the time-wise evaluation scenarios on the accuracy of NMT-based models. 




\paragraph{\textbf{\underline{Approach}}}
To answer this RQ, we focus on two types of evaluation scenarios: time-wise and time-ignore.
In the time-wise evaluation scenario the training dataset is first sorted
in chronological order, ensuring that method pairs that happen earlier appear only in the training dataset, but do not appear in the testing dataset.
Likewise, method pairs that happen later appear only in the testing dataset, but do not appear in the training dataset, ensuring a realistic evaluation setting.
Thus, for the time-wise evaluation, the training/validation dataset consists of the method pairs during 2008 to 2019, while the testing dataset consists of the method pairs during 2020 to 2022.
On the other hand, the time-ignore evaluation scenario does not consider the temporal information of the method pairs (which is the case for prior studies ~\cite{tufano2018empirical,thongtanunam2022autotransform}).
Thus, for the time-ignore evaluation, the training/validation/testing dataset consists of the method pairs that are randomly splitted without considering the temporal information.
Both types of evaluation scenarios are applied to our \ourapp~ and a baseline approach (i.e.,  AutoTransform~\cite{thongtanunam2022autotransform}).



\input{tables/RQ3_time_impacts}

\paragraph{\textbf{\underline{Results}}} Table~\ref{tab:RQ3_compare_time} presents the accuracy of our \ourapp~ and AutoTransform~\cite{thongtanunam2022autotransform} between the time-wise and time-ignore evaluation scenarios.

\textbf{Both NMT-based models produce optimistically higher accuracy in the time-ignore evaluation scenario (non-realistic) than in the time-wise evaluation scenario (realistic).}
Table~\ref{tab:RQ3_compare_time} shows that, at a Beam size of 15, for our \ourapp, the time-ignore evaluation scenario (33\% of PP) optimistically inflates the perfect predictions by 32\% when compared to the time-wise evaluation scenario (25\% of PP).
Similarly to \ourapp, the time-ignore evaluation scenario on AutoTransform (43\% of PP) optimistically inflates the perfect predictions by 290\% when compared to the time-wise evaluation scenario (11\% of PP).
This finding suggests that researchers should consider time-wise evaluation scenarios in the future.  


\begin{table}[t]
  \centering
  \caption{(RQ5.1) The accuracy of our \ourapp~when considering the \#All dataset.}
    \begin{tabular}{llrrr}
    \toprule
    \textbf{Dataset} & \multicolumn{1}{c}{\textbf{PP/Total}} & \multicolumn{1}{c}{\textbf{PP\%}}  \\
    \midrule
    \textbf{\ourapp} & 4,188/43,714 & 14\%  \\
    \textbf{\textsc{AutoTransform}} & 2,690/43,714 & 6\%  \\
    \bottomrule
    \end{tabular}%
  \label{tab:RQ2_overall_performance}%
\end{table}%


\subsection*{\textbf{(RQ5) \rqfive}}

\paragraph{\textbf{\underline{Motivation}}}
Following Tufano~\ea~\cite{tufano2019learning}, our experiment in RQ1-RQ4 is based on the small method pairs, containing fewer than 50 tokens in a method and fewer than 5 changed tokens between versions).
While our \ourapp~is able to correctly recommend code updates for Android apps (25\%PP at Beam=15), little is known about the accuracy of our \ourapp~on pairs of larger method and on larger updates (\#changed tokens between versions of a method).
Thus, we formulate this RQ to investigate the impact of the method size and the update size on the accuracy of our \ourapp.

\paragraph{\textbf{\underline{Approach}}}
To answer this RQ, we use the \#All dataset consisting of 209,346 method pairs. 
% Then, the \#All dataset is sorted in a chronological order.
The \#All dataset is sorted in a chronological order.
Then, we split the \#All dataset into training (136,932 method pairs during 2008-2019), validation (34,234 method pairs during 2008-2019), and testing (43,714 method pairs during 2020-2022) sets.
Then, both \ourapp~and AutoTransform are trained, validated, and tested, accordingly.
We note that we do not incorporate Tufano~\ea's approach~\cite{tufano2019learning} in this RQ, since the RNN-based approach is known to be computationally expensive, limiting its model training ability on our large dataset (i.e., 209,346 method pairs).
For our \ourapp, we further analyze the perfect predictions according to the method size (\#tokens in the initial version) and the update size (\#changed tokens between two versions) at the beam size of 15.


\paragraph{\textbf{\underline{Results}}}
Table~\ref{tab:RQ2_overall_performance} presents the accuracy of \ourapp~and AutoTransform when considering the \#All datasets.

\textbf{When considering all method pairs, our \ourapp~ achieves 133\% higher perfect predictions than the baseline approach.}
Table~\ref{tab:RQ2_overall_performance} shows that, when training and testing on any size of methods, our \ourapp~ still achieves a perfect prediction of 14\%.
On the other hand, the baseline approach only achieves a perfect prediction of 6\%, demonstrating an improvement of 133\% for \ourapp~over the baseline approach.
This indicates that, despite the method size (\#tokens) and update size (\#updated tokens) are much larger, our \ourapp~ still perform better than the baseline approach.


\input{tables/RQ4_token_size_compare}

\textbf{Nevertheless, our \ourapp~is less accurate when they are applied to a larger size of methods with a larger number of updated tokens.}
Table~\ref{tab:RQ4_token_length} shows that the accuracy of our \ourapp~ depends on the size of the method size and its update size.
Importantly, Table~\ref{tab:RQ4_token_length} shows that, at the small size of methods (i.e., Method size less than 50) and updates (i.e., \#Updated Tokens less than 5), our \ourapp~achieves the perfect prediction of 44\%, which is much higher than the overall accuracy (i.e., 25\%).
On the other hand, the perfect prediction is substantially decreased to less than 29\% when the method size is increased (i.e., Method size larger than 50), and to less than 11\% when the update size is increased (i.e., \#Updated Tokens more than 5).
Thus, this finding suggests an opportunity for future researchers to address this challenge.


\textbf{Interestingly, our \ourapp~is more accurate on the \#Small dataset when it is trained on the \#All dataset which includes a larger size of methods and a larger number of updated tokens.}
Table~\ref{tab:RQ4_token_length} shows that, when the model is trained on the \#All dataset and tested on the \#Small dataset (i.e., method size less than 50 and \#Updated Tokens less than 5), our \ourapp~achieves the perfect prediction of 44\%, which is higher than the 25\% (see Table~\ref{tab:RQ1compare}) when the model is trained on the small dataset.
Nevertheless, \ourapp becomes less accurate (0\%-11\%) when the method size is larger and the number of updated tokens is higher, highlighting a potential research opportunity for future researchers to improve the model performance for the more complex code updates.


==> results/5_result.tex <==
\section{Experimental Results}
\label{sec:results} 

In this section, we present approaches and results with respect to our five research questions.

\input{tables/RQ1_compare_with_baseline}

\subsection*{\textbf{(RQ1) \rqone}}
% \pick{We also have a result for efficiency. Should RQ be adjusted to include efficiency?}
\paragraph{\textbf{\underline{Motivation}}}
We formulate this RQ to investigate the accuracy of our \ourapp~(Abs+BPE+ Transformer) in the context of code updates in Android apps, when comparing to the two baseline approaches for code transformation.


% In this study, we propose \ourapp~ to automatically recommend code changes for Android applications. 
% Unlike the prior approach~\cite{tufano2019learning}, we leverage BPE subword tokenization and transformer techniques to recommend future code changes.
% As previously stated, code update recommendation for Android applications has not yet been empirically investigated.
% Therefore, we collect a set of code updates from 3,195 Android applications to construct four time-wise datasets to investigate the performance of our approach.
% Additionally, we compare our approach to one of the competitive baseline approaches proposed by Tufano et al.~\cite{tufano2019learning}.
% We formulate this RQ to evaluate whether our \ourapp~ can recommend future code updates by learning the existing code updates.
% To ensure the generated code is relevant and accurate, we evaluate our approach's model performance.
% We aim to empirically assess whether our approach is an effective approach to learn continues code evolution.
% As was mentioned in the previous chapters, there is no known empirical research that has focused on exploring code transformation learning under the code evolution scenario. 
% As previously stated, code transformation learning in the context of code evolution has not yet to be empirically investigated.
% Therefore, we use the collected datasets of evolved method pairs to investigate the performance of our approach.
% Additionally, we compare our approach to one of the competitive baseline approaches proposed by Tufano et al.~\cite{tufano2019learning}.

\paragraph{\textbf{\underline{Approach}}}
To answer this RQ, we evaluate the accuracy of our \ourapp~ and the baseline approaches based on the percentage of Perfect Predictions (\%PP). %, BLEU, and CodeBLEU.
Similar to prior studies~\cite{tufano2019learning,thongtanunam2022autotransform}, we leverage a beam width ($k$) of 1, 5, 10, 15 to generate $k$ candidate code updates. 
To quantify the magnitude of the improvement for our \ourapp, we compute a percentage improvement of the perfect predictions rate using a calculation of $\frac{(\#PP\%_\mathrm{our} - \#PP\%_\mathrm{baseline})\times 100\%}{\#PP\%_\mathrm{baseline}}$.
In addition, we also compare our \ourapp{} with the baseline approaches based on CodeBLEU.

To evaluate the efficiency of our \ourapp, we measure the training time of each approach.
Then, we compare the average training time of our \ourapp~ and the two baselines based on the same size of training data with the same training steps.
We run the experiments on the same machine with an AMD Ryzen 9 5950X CPU, 64 GM of RAM and an NVIDIA GeForce RTX 3090 GPU.
 
Note that since the RNN architecture used by the baseline approaches~\cite{tufano2019learning} is computationally-expensive, their approaches were evaluated using small methods (i.e., fewer than 50 tokens in a method and fewer than 5 changed tokens between versions).
% Their approaches are evaluated on the context of small methods only.
Thus, similar to prior studies~\cite{tufano2019learning, thongtanunam2022autotransform}, this RQ will focus on the context of small methods.
For each approach, the model is trained on the training dataset of small methods and tested on the testing dataset of small methods.
We will further evaluate our \ourapp{} based on the whole dataset in RQ5.
% To ensure that our evaluation is under a realistic time-wise evaluation scenario, the instances are first sorted in a chronological order.
% This allows us to ensure that instances that appear later in the testing dataset will not appear in the training dataset.
% Similarlly, instances that earlier appear in the training dataset will not appear later in the training dataset.


% Then, we compare \%Perfect Predictions of our~\ourapp{} with the two baseline approaches as follows:

% \begin{enumerate}
%     \item Tufano~\ea~\cite{tufano2019learning} is an NMT-based code transformation approach using code abstraction with RNN-based NMT architecture.
%     \item AutoTransform~\cite{thongtanunam2022autotransform} is an NMT-based code transformation approach using BPE~\cite{sennrich2015neural} with a vanilla transformer architecture~\cite{vaswani2017attention}.
% \end{enumerate}




% To answer this RQ, we evaluate how well our approach can recommend code updates given the pre-version of methods, comparing against Tufano \ea~\cite{tufano2019learning} approach.
% We trained \kla{try to use present tense} the two approaches on the same training dataset and generate updated methods in the testing dataset (i.e., Original\_small and Abstraction\_version).
% We leverage the BPE approach to perform a subword-level tokenization.
% For each recommendation, we output the best-k candidates to compare the performance (i.e., beam size =[1,5,10,15]) and calculate the number of Perfect Predictions(PP) and the perfect prediction rate (PP\%).
% Addtionally, we examine the training time required by \ourapp~ and the Tufano \ea~ approach.

\paragraph{\textbf{\underline{Results}}}
% and Table~\ref{tab:RQ1timecompare} provides the experimental results of our \ourapp~ and the baseline approaches on two time-wise datasets.
\textbf{Our \ourapp~ achieves a perfect prediction of 25\%, which is 59\%\textasciitilde107\% higher than the baseline approaches.}
Table~\ref{tab:RQ1compare} presents the accuracy of our \ourapp~comparing to the baseline approaches.
% Table~\ref{tab:RQ1compare} reports the performance of our \ourapp~ and with two baselines.
We find that when beam size is set to 15, our \ourapp~ achieves perfect prediction for 1036 changed methods which accounts as 25\% of the changed methods.
The Tufano \ea~ approach achieves the perfect prediction for 651 changed methods (i.e., \%PP is 15\%).
Compared with the Tofano~\ea, our \ourapp~ achieves a 59\% performance improvement. 
The AutoTransform approach achieves the perfect prediction for 656 changed methods (i.e., \%PP is 11\%).
Compared with AutoTransform, our \ourapp~ achieves a 133\% performance improvement. 
When the size of beam search is {1,5, or 10}, the perfect predictions of \ourapp~ improve by 73\%\textasciitilde107\% compared with the approach of Tufano \ea~.
These observations demonstrate that our \ourapp~ outperforms Tufano \ea~ and AutoTransform to generate a perfect prediction by a large margin. 

Table~\ref{tab:RQ1compare} also show that our \ourapp{} also achieve CodeBLEU higher than the baseline approaches.
When the beam size is set to 15, our \ourapp{} achieves CodeBLEU of 0.902 while the baseline approaches achieve CodeBLEU of 0.664 (Tufano) and 0.893 (AutoTransform).
The results are also similar when the beam size is {1, 5, 10}.
These results indicate that on average across all methods in the testing data, our \ourapp{} can generate code updates more similar to the actual code updates than the baseline approaches.


\textbf{Our \ourapp~ achieves a higher efficiency for recommending code updates compared with the Tufano~\ea~approach and AutoTransform.}
Table~\ref{tab:RQ1timecompare} shows the computational time of our \ourapp{} and the baseline approaches.
As shown in Table~\ref{tab:RQ1timecompare}, \ourapp~ takes about 117 minutes to train a model, while the approach of Tufano \ea~ takes 223 minutes and AutoTransform takes 140 minutes.
The result shows that our \ourapp~ can save 16\% - 50\% computational time when training a model on the small dataset. 
The higher efficiency of our \ourapp~has to do with our Transformer-based architecture, which processes the entire input sequences at once in a highly parallel fashion. 
In contrast, the RNNs-based models used by Tufano~\ea~\cite{tufano2019learning} needs to process the input sequence in order, which is less efficient as showed in Table~\ref{tab:RQ1timecompare}.

% \yonghui{Do we need to mention why higher efficiency than AutoTransform?}
% \kla{may be no because both autoupdate and autotransform use the same architecture, but we do not have reason to support why autoupdate is faster than autotransform}
% \pick{Please a short discussion why it takes less time to compute? The vocab size is smaller?}


\begin{table}[htbp]
  \centering
  \small
  \caption{Computational time of \ourapp~ and the baseline approaches.}
    \begin{tabular}{lrrr}
    \toprule
    \textbf{ Model } & \multicolumn{1}{c}{\textbf{ \ourapp }} & \multicolumn{1}{c}{\textbf{ Tufano \ea }} & \multicolumn{1}{c}{\textbf{ AutoTransform }} \\
    \midrule
    \textbf{Time cost} & 117 min & 233 min & 140 min \\
    \textbf{Improvement} &       & -50\% & -16\% \\
    \bottomrule
    \end{tabular}%
  \label{tab:RQ1timecompare}%
\end{table}%





\subsection*{\textbf{(RQ2) \rqtwo}}

\paragraph{\textbf{\underline{Motivation}}} 
Tufano~\ea~\cite{tufano2019learning} suggested that code abstraction could substantially reduce the size of vocabularies. 
However, Thongtanunam~\ea~\cite{thongtanunam2022autotransform} argue that, when code abstraction is used together with word-level tokenization, the approach may generate an excessively large number of vocabularies.
Different from prior work, our \ourapp~leverages both code abstraction and BPE in order to preserve existing tokens that will be appeared in the updated version and generate new tokens that do not exist in the prior version.
Thus, we formulate this RQ to investigate the benefits of our tokenization approaches for our \ourapp.

\paragraph{\textbf{\underline{Approach}}}
To answer this RQ, we conduct an ablation study to evaluate the following four variants of our \ourapp~ using different tokenization approaches:

\begin{itemize}
    \item Abs+BPE+Transformer (our \ourapp).
    \item BPE+Transformer (AutoTransform~\cite{thongtanunam2022autotransform}).
    \item Abs+Transformer (Abs is used in Tufano~\ea~\cite{tufano2019learning}).
    \item Word-level+Transformer.
\end{itemize}
Similar to RQ1, for each approach, the model is trained on the training dataset of small methods and tested on the testing dataset of small methods.
Finally, we evaluate the accuracy of these variants using the same evaluation measure (i.e., \% Perfect Predictions).


% To answer this RQ, we conduct an experiment of different code tokenization approach with the same Transformer architecture. 
% Specifically, we extend our approaches to evaluate the following four variants: word-based tokenization (i.e., 1-gram word level tokenization which splits raw code by white space), only code abstraction, only BPE subword toknization, and code abstraction + BPE. 
% After that, we build the Transformer to test the prediction performance. 
% We evaluate the accuracy (i.e., perfect prediction rate) under different beam sizes.

\begin{figure}[t]
  \centering
  \includegraphics[width=0.8\columnwidth]{results/RQ2.pdf}
  \caption{(RQ2) The perfect prediction of the different tokenization approaches.}
  \label{fig:RQ2Evaluation_tokenization}
\end{figure}


\paragraph{\textbf{\underline{Results}}}
Figure~\ref{fig:RQ2Evaluation_tokenization} presents the accuracy of different code tokenization approaches of our \ourapp.

\textbf{Our tokenization approach (Abs + BPE) gains benefits at least 17\% by using both code abstraction and BPE for recommending code updates.}
Figure~\ref{fig:RQ2Evaluation_tokenization} shows that our approach (Abs + BPE) achieves the highest accuracy regardless of the size of beam search.
Specifically, at the beam size of 15, our approach achieves the perfect prediction of 25\%.
On the other hand, code abstraction alone achieves the perfect prediction of 23\%, while BPE alone achieves the perfect prediction of 11\%.
The higher accuracy of using code abstraction only than using BPE only is different from Thongtanunam~\ea~\cite{thongtanunam2022autotransform} who found that BPE is better than code abstraction, highlighting the importance of this work that findings from existing NMT-based code transformation studies are not generalized to NMT-based code update recommendations.
We suspect that BPE works well for the context of code review, since there are a large number of newly-introduced code tokens.
In contrast, for Android apps, the proportion of newly-introduced code tokens is smaller, demonstrating that code abstraction only performs better than BPE only.
Nevertheless, our finding confirms that the combination of using both Abs and BPE used by our \ourapp~outperforms both Abs alone and BPE alone.


% However, we observe that the accuracy decreases to 23\% when only leveraging code abstraction and decreases to 11\% when only using BPE subword tokenization. 
% When both the code abstraction and BPE tokenization are not applied, the transformer architecture only obtains 2\% accuracy.


\subsection*{\textbf{(RQ3) \rqthree}}

\paragraph{\textbf{\underline{Motivation}}}
Prior studies proposed various approaches to automatically update Android apps, yet for specific types of code updates.
For example, 
Lamothe et al.~\cite{lamothe2020a3} focus on updating Android API migrations.
Zhao et al.~\cite{zhao2022towards} focus on updating compatibility issues.
% However, existing approaches are .
Indeed, there exist multiple types of code updates~\cite{Conventional-commit-types} associated with Android apps (e.g., \textit{Fixing Bug} or \textit{Refactoring Method}).
Thus, we set out this RQ to qualitatively evaluate \ourapp{} in terms of the types of code updates that can be recommended by our \ourapp. 
% Thus, we formulate this RQ to manually investigate the types of code updates that are correctly 

% To this goal, we focus only on the successfully predicted code transformations generated from the model in RQ1 and manually analyze the prefect predictions in the testing data.


% After obtaining the perfect predictions, 
% we aim to qualitatively analyze the types of code changes that our model is able to generate.
% The purpose of this section is to provide an in-depth examination of the sorts of code changes that our model is capable of generating, especially for perfect predictions.
% Although the previous several RQs have answered our \ourapp~can recommend code changes for Android applications, little is known about what kinds of code updates can be recommended by the model (e.g., bug fix). 
% While the last four RQs established that our \ourapp~can recommend code changes for Android applications, little is known about how these recommended codes impact the application (e.g., bug fix). 

\paragraph{\textbf{\underline{Approach}}}
To answer this RQ, we analyze the 277 updated methods that are correctly recommended by our \ourapp{} when using the beam size of 1 from RQ1.
% ~(i.e., the group of 7\% perfect predictions at the beam size of 1).
To do so, we manually classify updated methods into various types of code updates. 
% \lili{The next sentence is not correct.}
We use the high-level taxonomy of the conventional commit types~\cite{Conventional-commit-types} and Tufano~\ea's approach~\cite{tufano2019learning} for the types of code updates. 
To fully understand the purpose of code updates, we also use the commit messages associated with the studied updated methods. 
% For each of the method pairs, we collect the human-written commit log messages that are associated with that method pair.
% Commit messages are natural language descriptions of changes in source code written by software developers, which is often used to describe the intent of the code changes, e.g., "\emph{Fix integer division in floating-point contexts}".
The categorization process was performed by the first author and the results of coding were cross-checked by the third author to mitigate any potential bias in the categorization process.
Then, we calculate the inter-rater agreement between the categorization results from the two coders using a Cohen's kappa. 
The kappa agreement is 0.91 for the categorization process of the 277 perfect predictions, demonstrating the high agreement (i.e., almost perfect) between two raters~\cite{cohen1968weighted}.
% that the agreement of our manual categorization is almost perfect.
% \pick{It would be great if we can report the Cohen kappa for the aggreement level.}
% \kla{Yue, prepare a spreadsheet of these 277 to your friend to privately do the coding. Then, we will compute the Cohen kappa to see the agreement \footnote{\url{https://scikit-learn.org/stable/modules/generated/sklearn.metrics.cohen_kappa_score.html}}}
% \yue{cohen kappa score 0.91, will update the description today morning}
% The results are then cross-checked by another author to mitigate any potential bias in the coding process.


% We follow the taxonomy of code updates by \cite{tufano2019learning} and \cite{Conventional-commit-types} to categorize the perfect predictions that our \ourapp~ recommends.
% Since there is no specific taxonomy for code updates of Android applications, we also 


\paragraph{\textbf{\underline{Results}}} 
% \kla{@Li, can check below?}
Table~\ref{tab:rq5} sumarizes the types of code updates that  our \ourapp{} can achieve concerning a perfect prediction with a beam size of 1.\footnote{Due to the page limit, the complete classification results are available in the GitHub repository.}

\textbf{Our \ourapp~ can recommend nine types of code updates for Android apps, e.g., 26\% perfect predictions for fixing bug and 22\% perfect predictions for adding new features.}
As Table~\ref{tab:rq5} shows, we summarize nine types of code updates.
\textit{Fixing bug} and \textit{Adding New Feature} are the most common types of code updates that \ourapp{} can recommend (i.e., 26\% for \textit{Fixing Bug} and 22\% for \textit{Adding New Feature}).
% \pick{If the space is available, we can add actual examples of code update (like Tufano et al paper). Then further elaborate what kinds of bug fixes and features are in the code update (similar to what we discuss for Maintaining Android OS Compatibility).}
% \lili{I agree, showing a concrete example would be great. The example should not be very simple (but also not very complicated) and should also include the commit message indicating why it is grouped in that category.}
Also, our \ourapp{} can recommend maintainability-related code updates for Android applications (e.g., \textit{Refactoring Method} and \textit{Adjusting Build} for Android applications).
% Some common code updates, like bug fixes, new features, and code refactoring, are included in the perfect predictions by our \ourapp.
% For several typical code updates, our tool is capable of having perfect predictions (e.g., bug fixes, new features, code refactoring, etc.).
% Besides that, we also find some specific code updates for Android applications.
% Android developers update the source code to adapt to the new version of Android OS (i.e., Android OS Maintenance).
% At the same time, Android applications usually include third-party libraries to increase performance and reuse functionalities. 
% When the third-party libraries update, Android developers need to update the source code to support the new libraries. 
% Some of the code updates are also specific to Android app updates.
Additionally, some of the code updates are related to external code updates (e.g., third-party libraries and Android OS).
For example, Android developers update the source code to adapt to the release of new version of Android OS (i.e., Maintaining Android OS Compatibility).
% Another example is that Android developers need to update the source code to accommodate the new third-party libraries (i.e., \pick{what type?}). 
These results suggest that our \ourapp{} can recommend various types of code updates, demonstrating the potential impact of our \ourapp{} in real-world usage scenarios.

% \kla{if you could provide example images of a code snippet with a commit message for 'bug fix' or something exciting, we may get 10 pages... just more pictures and some more discussion for RQ3 to make it richer. you can discuss with me via Slack if this example is clear or not.}
% \yue{I want to give example for code update, But I only stored the abstracted code before we plan to add the code abstraction as one of our step. I don't store the mapping to reconstruct the original code and I think it is not good to put the abstraction version}

% We also find certain unique code updates for Android applications due to external causes.
% Android developers update the source code to adapt to the release of new version of Android OS (i.e., Android OS Maintenance).
% Additionally, third-party libraries are widely utilised in Android applications to improve efficiency and functionality reuse. 
% When the third-party libraries update, Android developers need to update the source code to accommodate the new libraries. 

% \textbf{Bug fixes and new features are the two most accurately types of code updates by our ~\ourapp.}
% Table~\ref{tab:rq5} presents that our \ourapp recommend the most code changes related to bug fixes, with 26 percent. 
% We observe that 68 perfect prediction (25\%) are related to updating new features for the Android applications. 

\input{tables/RQ5}

\subsection*{\textbf{(RQ4) \rqfour}}

\paragraph{\textbf{\underline{Motivation}}}
Source codes gradually evolves over time.
Thus, evaluation scenarios for NMT-based code transformation should take into consideration temporal information. 
Prior studies~\cite{pornprasit2021jitline,cabral2019class, pendlebury2019tesseract, de2021compromised} raised concerns that random data splitting (which has been widely-used in previous NMT-based code transformation approaches~\cite{tufano2018empirical,thongtanunam2022autotransform}) may not be realistic (i.e., time-ignore), ignoring the temporal information that must be considered.
Yet, little is known about the impact of the time-wise evaluation scenarios on the accuracy of NMT-based models. 

% Several prior studies have raised concerns that in non-stationary contexts (e.g., Android malware detection), if time-wise splits are not considered, then the experimental results may be inflated due to concept drift (i.e., changes in the data distribution)~\cite{cabral2019class, pendlebury2019tesseract, de2021compromised}.
% Yet, little is known about whether concept drift exerts influence on automated code transformation or not.
% To the best of our knowledge, no previous studies in code-based tasks have investigated the impacts of concept drift.
% This study provides the first assessment of the concept drifts in automated code transformation.
% Here we aim to specifically evaluate the effectiveness of our \ourapp~ to automatically recommend code updates.
% Thus, we formulate this RQ to conduct a comparison experiment to understand the impacts of time-splits of the datasets. 
% We investigate the code transformation performance on two time-wise dataset in previous two RQs.
% To better the impacts of time splits, we evaluate our approach on the collected dataset with more types of time splits.
% We compare our approach on temporally inconsistent datasets and temporally consistent datasets (i.e., realistic settings).



\paragraph{\textbf{\underline{Approach}}}
To answer this RQ, we focus on two types of evaluation scenarios: time-wise and time-ignore.
In the time-wise evaluation scenario the training dataset is first sorted
in chronological order, ensuring that method pairs that happen earlier appear only in the training dataset, but do not appear in the testing dataset.
Likewise, method pairs that happen later appear only in the testing dataset, but do not appear in the training dataset, ensuring a realistic evaluation setting.
Thus, for the time-wise evaluation, the training/validation dataset consists of the method pairs during 2008 to 2019, while the testing dataset consists of the method pairs during 2020 to 2022.
On the other hand, the time-ignore evaluation scenario does not consider the temporal information of the method pairs (which is the case for prior studies ~\cite{tufano2018empirical,thongtanunam2022autotransform}).
Thus, for the time-ignore evaluation, the training/validation/testing dataset consists of the method pairs that are randomly splitted without considering the temporal information.
Both types of evaluation scenarios are applied to our \ourapp~ and a baseline approach (i.e.,  AutoTransform~\cite{thongtanunam2022autotransform}).

% we reconstruct one time-ignore datasets to compare the performance of automated code update recommendations.
% To perform a fair comparison, we follow the same size of training, validation and testing sets as the time-wise splits.  
% To perform a fair comparison, we follow the same size of training, and validation, along with testing sets as the time-wise splits.
% Specifically, we firstly randomly shuffle the \textit{Original\_small} and \textit{Abstract\_small} datasets, and split the dataset into training, validation and testing sets.
% Specifically, we firstly shuffle the small datasets at random, and further split each of them into training, validation and testing sets, respectively.
% Following that, we obtain the time-ignore experimental datasets called {small\_random} which disregards the temporal distribution of updated method pairs.
% We extend our experiment to test the performance of our \ourapp~ on these two time-ignore datasets. 
% We extend our experiment to investigate how well our \ourapp~ performs on these two types of datasets (i.e., time-wise dataset and time-ignore dataset).

\input{tables/RQ3_time_impacts}

\paragraph{\textbf{\underline{Results}}} Table~\ref{tab:RQ3_compare_time} presents the accuracy of our \ourapp~ and AutoTransform~\cite{thongtanunam2022autotransform} between the time-wise and time-ignore evaluation scenarios.

\textbf{Both NMT-based models produce optimistically higher accuracy in the time-ignore evaluation scenario (non-realistic) than in the time-wise evaluation scenario (realistic).}
Table~\ref{tab:RQ3_compare_time} shows that, at a Beam size of 15, for our \ourapp, the time-ignore evaluation scenario (33\% of PP) optimistically inflates the perfect predictions by 32\% when compared to the time-wise evaluation scenario (25\% of PP).
Similarly to \ourapp, the time-ignore evaluation scenario on AutoTransform (43\% of PP) optimistically inflates the perfect predictions by 290\% when compared to the time-wise evaluation scenario (11\% of PP).
This finding suggests that researchers should consider time-wise evaluation scenarios in the future.  
% \kla{Yue to add percentage XX}

%  the perfect predictions of  based on 

% On the other hand, we observe that our \ourapp~ achieves a higher prediction performance when the unrealistic temporal split is introduced in the evaluation dataset. 
% This finding indicates that the performance of recommending code updates is related to the temporal distribution between the training and testing samples in the experimental datasets.
% Unrealistic train-test splits drastically exaggerate the prediction performance (i.e., from 3\% to 30\% accuracy).
% This disparity indicates that the traditional evaluation approaches (i.e., time-ignore evaluation) are unrealistic for measuring the performance of real-world code-related tasks.




% Unrealistic temporal distribution of the datasets (i.e., concept drift) exaggerates the code update recommendation performance.
% Table~\ref{tab:RQ3_compare_time} presents that AutoTransform achieves 3\% accuracy when beam size is one under the time-wise setting. 
% However, when randomly splitting the training and testing data (i.e., under the time-ignore scenario), AutoTransfrom can achieve 30\% accuracy, which is 900\% higher than the perfect predictions achieved under the time-wise setting.
%Similarly, AutoTransform can achieve a higher BLEU and CodeBLEU score when the unrealistic temporal split is introduced in the evaluation dataset. 
% On the other hand, we observe that our \ourapp~ achieves a higher prediction performance when the unrealistic temporal split is introduced in the evaluation dataset. 
% This finding indicates that the performance of recommending code updates is related to the temporal distribution between the training and testing samples in the experimental datasets.
% Unrealistic train-test splits drastically exaggerate the prediction performance (i.e., from 3\% to 30\% accuracy).
% This disparity indicates that the traditional evaluation approaches (i.e., time-ignore evaluation) are unrealistic for measuring the performance of real-world code-related tasks.
% We encourage the community to focus on building a time-wise evaluation for the code-related tasks to provide a reliable experimental analysis.   

% \kla{likely drop below}
% \textbf{The accuracy of Our \ourapp~ gradually decreases over time.}
% As shown in Table~\ref{tab:RQ3_compare_time}, \ourapp~ achieves 25\% accuracy on the whole testing data set (i.e., samples from 2020 to 2022) under time-wise scenarios, which is much lower than when splitting training and testing data randomly.
% We further analyze the performance of our \ourapp with respect to the timestamps of method pairs under the time-wise evaluation, as presented in Figure~\ref{fig:RQ3_time_decay}. 
% When the beam size is set to 15, we observe that \ourapp~ achieves 25.1\% accuracy on 2020 data, 24.5\% accuracy on 2021 data, and 21.9\% on 2022 data.
% Similarly, Figure~\ref{fig:RQ3_time_decay} shows that the prediction performance of \ourapp~ gradually decreases over time. 
% In the AI community, this problem is also known as dataset shift or concept drift~\cite{gama2014survey, pendlebury2019tesseract}.
% Indeed, our observation demonstrates that concept drift is problematic in code update recommendations, and we encourage our community to realize the concept drift problem and study how to integrate expert knowledge into concept drift handling.

% \begin{figure}[t]
%   \centering
%   \includegraphics[width=\columnwidth]{figures/RQ3_time_decay.pdf}
%   \caption{(RQ4) The perfect prediction of our \ourapp~ over time.}
%   \label{fig:RQ3_time_decay}
% \end{figure}


\begin{table}[t]
  \centering
  \caption{(RQ5.1) The accuracy of our \ourapp~when considering the \#All dataset.}
    \begin{tabular}{llrrr}
    \toprule
    \textbf{Dataset} & \multicolumn{1}{c}{\textbf{PP/Total}} & \multicolumn{1}{c}{\textbf{PP\%}}  \\
    \midrule
    \textbf{\ourapp} & 4,188/43,714 & 14\%  \\
    \textbf{\textsc{AutoTransform}} & 2,690/43,714 & 6\%  \\
    \bottomrule
    \end{tabular}%
  \label{tab:RQ2_overall_performance}%
\end{table}%


\subsection*{\textbf{(RQ5) \rqfive}}

\paragraph{\textbf{\underline{Motivation}}}
Following Tufano~\ea~\cite{tufano2019learning}, our experiment in RQ1-RQ4 is based on the small method pairs, containing fewer than 50 tokens in a method and fewer than 5 changed tokens between versions).
While our \ourapp~is able to correctly recommend code updates for Android apps (25\%PP at Beam=15), little is known about the accuracy of our \ourapp~on pairs of larger method and on larger updates (\#changed tokens between versions of a method).
Thus, we formulate this RQ to investigate the impact of the method size and the update size on the accuracy of our \ourapp.

\paragraph{\textbf{\underline{Approach}}}
To answer this RQ, we use the \#All dataset consisting of 209,346 method pairs. 
% Then, the \#All dataset is sorted in a chronological order.
The \#All dataset is sorted in a chronological order.
Then, we split the \#All dataset into training (136,932 method pairs during 2008-2019), validation (34,234 method pairs during 2008-2019), and testing (43,714 method pairs during 2020-2022) sets.
Then, both \ourapp~and AutoTransform are trained, validated, and tested, accordingly.
We note that we do not incorporate Tufano~\ea's approach~\cite{tufano2019learning} in this RQ, since the RNN-based approach is known to be computationally expensive, limiting its model training ability on our large dataset (i.e., 209,346 method pairs).
For our \ourapp, we further analyze the perfect predictions according to the method size (\#tokens in the initial version) and the update size (\#changed tokens between two versions) at the beam size of 15.


% we seek to ascertain factors that affect the accuracy of our \ourapp.
% To better analyze the performance,
% Specifically, we train our \ourapp~ on the whole Original and Abstraction dataset. Then we further analyze the performance of our \ourapp~ with respect to the updated degree and the method length.
% We perform a further investigation to the analyze the performance of our \ourapp~ with respect to the updated degree and the method length.



% \kla{Yue Revised here} Table~\ref{tab:RQ2_overall_performance} presents the experimental results of our \ourapp~ on the large \textit{Original} and \textit{Abstract} datasets.


\paragraph{\textbf{\underline{Results}}}
Table~\ref{tab:RQ2_overall_performance} presents the accuracy of \ourapp~and AutoTransform when considering the \#All datasets.

\textbf{When considering all method pairs, our \ourapp~ achieves 133\% higher perfect predictions than the baseline approach.}
Table~\ref{tab:RQ2_overall_performance} shows that, when training and testing on any size of methods, our \ourapp~ still achieves a perfect prediction of 14\%.
On the other hand, the baseline approach only achieves a perfect prediction of 6\%, demonstrating an improvement of 133\% for \ourapp~over the baseline approach.
This indicates that, despite the method size (\#tokens) and update size (\#updated tokens) are much larger, our \ourapp~ still perform better than the baseline approach.




% \kla{present the results without Table?, since we didn't talk about BLEU and CodeBLEU. Please revise below.} \yue{done}
% \textbf{Our \ourapp~ can achieve good performance on large-scale of dataset}
% Table~\ref{tab:RQ2_overall_performance} show the evaluation results of our \ourapp~ on the large datasets when the beam size is set to 15.
% When applying AutoTransform, we observe 2690 perfect predictions with 6\% perfect prediction rate.
% When applying \ourapp, the model achieves 4188 perfect predictions with 14\% perfect prediction rate.
% We train our \ourapp~ using a large dataset, which contains
% the methods with large token sizes and token changes.
% Table~\ref{tab:RQ2_overall_performance} illustrates the evaluation results of our \ourapp~ on huge datasets with beam size set to 15.
% When applying AutoTransform, we observe 2690 perfect predictions with 6\% perfect prediction rate.
% The model achieves 4188 perfect predictions with a 14\% perfect prediction rate while using \ourapp~.
% Our \ourapp~ could increase the prediction accuracy by 133\% for larger method size and higher change complexity. 



% \textbf{For the small method size, our \ourapp~trained on datasets with all size achieves X\% higher perfect predictions than our \ourapp~trained on datasets with small methods only.}
\input{tables/RQ4_token_size_compare}

\textbf{Nevertheless, our \ourapp~is less accurate when they are applied to a larger size of methods with a larger number of updated tokens.}
Table~\ref{tab:RQ4_token_length} shows that the accuracy of our \ourapp~ depends on the size of the method size and its update size.
Importantly, Table~\ref{tab:RQ4_token_length} shows that, at the small size of methods (i.e., Method size less than 50) and updates (i.e., \#Updated Tokens less than 5), our \ourapp~achieves the perfect prediction of 44\%, which is much higher than the overall accuracy (i.e., 25\%).
On the other hand, the perfect prediction is substantially decreased to less than 29\% when the method size is increased (i.e., Method size larger than 50), and to less than 11\% when the update size is increased (i.e., \#Updated Tokens more than 5).
Thus, this finding suggests an opportunity for future researchers to address this challenge.
% The accuracy decrease for larger methods and complex updates has to do with the window size of the Transformer architecture (i.e., limited to 512 tokens). 
% For any vulnerable functions with greater than 512 tokens, such extra tokens will be truncated and will not be processed and learned by the models, leading to the negative impact on the accuracy of our \ourapp.
% Thus, \emph{future researchers should further explore techniques that can handle larger functions (i.e,. the functions with more than 512 tokens).}


\textbf{Interestingly, our \ourapp~is more accurate on the \#Small dataset when it is trained on the \#All dataset which includes a larger size of methods and a larger number of updated tokens.}
Table~\ref{tab:RQ4_token_length} shows that, when the model is trained on the \#All dataset and tested on the \#Small dataset (i.e., method size less than 50 and \#Updated Tokens less than 5), our \ourapp~achieves the perfect prediction of 44\%, which is higher than the 25\% (see Table~\ref{tab:RQ1compare}) when the model is trained on the small dataset.
Nevertheless, \ourapp becomes less accurate (0\%-11\%) when the method size is larger and the number of updated tokens is higher, highlighting a potential research opportunity for future researchers to improve the model performance for the more complex code updates.
% We perform a further investigation to check the testing data based on the method length and the number of token changes.
% Table~\ref{tab:RQ4_token_length} presents the perfect predictions of our \ourapp~ with respect to the method size (\#tokens) and the update size (\#changed tokens between two versions).
% From Table~\ref{tab:RQ4_token_length}, our \ourapp~ achieve the best accuracy (i.e., 44\% perfect prediction rate) when the paired methods have less than 50 tokens and less than five updated tokens.
% However, When the number of updated tokens is less than five, our \ourapp~ only achieves a 10\% perfect prediction rate when the paired methods have greater than 200 tokens.
% The results prove that our \ourapp~ presents a substantial decrease on the prediction performance as the method length increase, 
% At the same time, our \ourapp~achieves perfect prediction of 10\%\textasciitilde44\% for code updates with less than five updated tokens, but the value is substantially reduced with more than five updated tokens.
% For example, when the method length is less than 50, the perfect prediction rate can drop from 44\% to 1\% as the number of updated tokens increases.
% Similarly, we also observe a BLEU score decrease from 0.916 to 0.312.
% These observations suggest that the update degree (measured by \#updated tokens) causes the negative impract on the accuracy of our \ourapp.



% Although our \ourapp~ achieves 4188 perfect predictions on the large dataset, the perfect prediction rate is much lower than that on the small dataset. 
% Specifically, our \ourapp~ achieves a 25\% perfect prediction rate when the dataset only contains methods with a small size.
% However, the accuracy decreases to 14\% when adding more complex method pairs with larger sizes and more complex updates.
% Thus, future researchers should further explore techniques that can handle difficult code updates.


% \kla{Yue, to update below}
% , providing a research opportunity for future researchers.

% \textbf{The accuracy of our \ourapp{} depends on the size of the vulnerable functions and its difficulty to repair.}
% Table~\ref{tab:discussion} shows that our \ourapp{} is most accurate for vulnerable functions that have less than 500 tokens and less than 20 repair tokens.
% Our \ourapp{} achieves the \%Perfect Prediction of 64\%-77\% for for vulnerable functions with less than 500 tokens, but the \%Perfect Prediction is substantially decreased to 32\% for vulnerable functions with greater than 500 tokens.
% The performance decrease for large functions (500+ tokens) has to do with the window size of the T5 architecture (i.e., limited to 512 tokens). 
% For any vulnerable functions with greater than 512 tokens, such extra tokens will be truncated and will not be processed and learned by the models, leading to the negative impact on the accuracy of our \ourapp.
% Thus, \emph{future researchers should further explore techniques that can handle larger functions (i.e,. the functions with more than 512 tokens).}


% This limitation has relation to the self-attention architecture of \ourapp~that the dot-product computation would grow quadratically when increasing the sequence length.
% However, the median of the input function length is only 280 in our testing data. 
% Therefore, our \ourapp~is still feasible to achieve high \% Perfect Predictions compared with existing baselines.
% \kla{michael explain here about 512 tokens window size}.

% In addition, the repair difficulty (measured by \#repair tokens in the vulnerability repair) is also impacting the accuracy of our \ourapp.
% We find that our \ourapp{} achieves the \%Perfect Prediction of 63\%-77\% for vulnerable repairs with less than 10 repair tokens, but the \%Perfect Prediction is substantially decreased to below 60\% for vulnerable repairs with greater than 10 repair tokens.
% Thus, \emph{future researchers should further explore techniques that can handle difficult repairs (i.e,. repairs with more than 20 repair tokens).} 











==> sections/similarity_compare.tex <==
\section{Threats to Validity}
\label{sec:threats}


==> tables/RQ5.tex <==
% Table generated by Excel2LaTeX from sheet 'NEWrq4'
\begin{table*}[t]
  \centering
  \caption{The distributions of the type of code updates.
  }
  \scriptsize
    \begin{tabular}{r l c c}
    \toprule
    \multicolumn{1}{c}{\textbf{Code Update Type}} & \multicolumn{1}{c}{\textbf{Description}} & \multicolumn{1}{c}{\textbf{Counts}} & \multicolumn{1}{c}{\textbf{Percentage}} \\
    \midrule
        \textbf{Fixing Bug} & A bug fix & 793 & 12.73\% \\
        \textbf{Adding New Feature} & Adding a new feature & 1331 & 21.37\% \\
        \textbf{Refactoring Method} & Restructuring existing code without changing its external behavior & 1004 & 16.12\% \\
        \textbf{Adjusting Build} & Changes that affect the build system or external dependencies & 1180 & 18.95\% \\
        \textbf{Maintaining Compatibility} & Updating code to resolve Android compatibility issues & 54 & 0.87\% \\
        \textbf{Improving Performance} & A code change that improves performance & 74 & 1.19\% \\
        \textbf{Optimizing Test Case} & Adding missing tests or correcting existing tests & 160 & 2.57\% \\
        \textbf{Altering Documentation} & Documentation only changes & 542 & 8.70\% \\
        \textbf{Other} & Other & 1089 & 17.49\% \\
        \bottomrule
    \end{tabular}%
  \label{tab:rq5}%
\end{table*}%



==> tables/newRQ2.tex <==
% Table generated by Excel2LaTeX from sheet 'NEWrq4'
\begin{table}[t]
  \centering
  
  \caption{(RQ2) The type of code updates that are correctly recommended}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{lcccccccc}
    \toprule
    \textbf{Code Update Type} & \multicolumn{1}{c}{\textbf{CodeT5}} & \multicolumn{1}{c}{\textbf{CodeT5+}} & \multicolumn{1}{c}{\textbf{CodeBERT}} & \multicolumn{1}{c}{\textbf{CodeGPT}} & \multicolumn{1}{c}{\textbf{UniXcoder}} & \multicolumn{1}{c}{\textbf{T5}} & \multicolumn{1}{c}{\textbf{AutoTransform }} & \multicolumn{1}{c}{\textbf{Tufano et al. }} \\
    \midrule
    \textbf{Fixing Bug} & 19\%  & 16\%  & 11\%  & 13\%  & 9\%   & 15\%  & 9\%   & 4\% \\
    \textbf{Adding New Feature} & 20\%  & 19\%  & 9\%   & 12\%  & 11\%  & 15\%  & 7\%   & 2\% \\
    \textbf{Refactoring Method} & 20\%  & 17\%  & 9\%   & 11\%  & 10\%  & 18\%  & 6\%   & 3\% \\
    \textbf{Adjusting Build} & 24\%  & 22\%  & 14\%  & 15\%  & 15\%  & 22\%  & 9\%   & 8\% \\
    \textbf{Maintaining Compatibility} & 6\%   & 13\%  & 6\%   & 7\%   & 9\%   & 11\%  & 7\%   & 6\% \\
    \textbf{Improving Performance} & 16\%  & 16\%  & 7\%   & 7\%   & 11\%  & 9\%   & 7\%   & 1\% \\
    \textbf{Optimizing Test Case} & 14\%  & 14\%  & 6\%   & 12\%  & 10\%  & 22\%  & 4\%   & 1\% \\
    \textbf{Altering Documentation} & 22\%  & 23\%  & 14\%  & 15\%  & 16\%  & 23\%  & 13\%  & 4\% \\
    \textbf{Other} & 12\%  & 16\%  & 7\%   & 6\%   & 8\%   & 9\%   & 5\%   & 2\% \\
    \midrule
    \textbf{Overall PP rate} & 19\%  & 19\%  & 10\%  & 12\%  & 11\%  & 17\%  & 8\%   & 4\% \\
    \bottomrule
    \end{tabular}}%
  \label{tab:newrq2summary_types}%
\end{table}%


==> tables/rq3_unsee_seen_distribution.tex <==
% Table generated by Excel2LaTeX from sheet 'time_simplify'
\begin{table}[t]
  \centering
  \caption{(RQ3) Distribution and Performance of CodeLMs on Seen vs Unseen Simplified Updates}
    \begin{tabular}{ccccc}
    \toprule
    \multirow{2}[2]{*}{\textbf{Approach}} & \multicolumn{2}{c}{\textbf{Time-aware}} & \multicolumn{2}{c}{\textbf{Time-ignore}} \\
          & \textbf{Seen} & \textbf{Unseen} & \textbf{Seen} & \textbf{Unseen} \\
    \midrule
    \textbf{CodeT5} & 43\%  & 10\%  & 71\%  & 20\% \\
    \textbf{CodeT5+} & 40\%  & 10\%  & 72\%  & 20\% \\
    \textbf{CodeBERT} & 26\%  & 4\%   & 60\%  & 11\% \\
    \textbf{CodeGPT} & 25\%  & 7\%   & 75\%  & 18\% \\
    \textbf{UniXcoder} & 24\%  & 6\%   & 74\%  & 20\% \\
    \textbf{T5} & 37\%  & 9\%   & 57\%  & 15\% \\
    \textbf{AutoTransform } & 21\%  & 3\%   & 65\%  & 12\% \\
    \textbf{Tufano et al. } & 9\%   & 2\%   & 15\%  & 4\% \\
    \midrule
    \textbf{Data Distribution} & \textbf{28\%} & \textbf{72\%} & \textbf{52\%} & \textbf{48\%} \\
    \bottomrule
    \end{tabular}%
  \label{tab:rq3_seen_unseen}%
\end{table}%


==> tables/table1_code_extraction_summary.tex <==
% Table generated by Excel2LaTeX from sheet 'summary_data'
\begin{table}[t]
  \centering
  \caption{Dataset summary \kla{merge this with Table 1 / to the right. need to mention how many apps. in the caption is fine.}}
    \begin{tabular}{lrrr}
    \toprule
    \textbf{Dataset} & \multicolumn{1}{c}{\textbf{\#Training}} & \multicolumn{1}{c}{\textbf{\#Validation}} & \multicolumn{1}{c}{\textbf{\#Testing}} \\
    \textbf{Original} &             136,932  &               34,234  &               43,714  \\
    \textbf{Small} &               19,638  &                 4,910  &                 6,227  \\
    \bottomrule
    \end{tabular}%
  \label{tab:section4_3_dataset_summary}%
\end{table}%



